Term Relevance Feedback for Contextual Named Entity Retrieval

We address the role of a user in Contextual Named Entity Retrieval (CNER), showing (1) that user identification of important context-bearing terms is superior to automated approaches, and (2) that further gains are possible if the user indicates the relative importance of those terms. CNER is similar in spirit to List Question answering and Entity disambiguation. However, the main focus of CNER is to obtain user feedback for constructing a profile for a class of entities on the fly and use that to retrieve entities from free text. Given a sentence, and an entity selected from that sentence, CNER aims to retrieve sentences that have entities similar to query entity. This paper explores obtaining term relevance feedback and importance weighting from humans in order to improve a CNER system. We report our findings based on the efforts of IR researchers as well as crowdsourced workers.

==> input/Research_Ideas.tex <==
over-specified and under-specified queries. 

Can a sentence with a marked entity be an alternative for a list question? 

Can a sentence with marked contextual words be an alternative for a list question? 

I argue that forming a question is hard, and our interactive system can let users form complex list questions. 

The context of the answer phrase that validates it as
an answer to the question is usually a small fraction
of the document it is embedded in \cite{Prager99theuse}.

Sometimes the expected answers have multiple attributes, e.g. Name four people from Massachusetts who were candidates for Vice-Presidents. Such attributes are translated into keywords that are used to retrieve passages or relevant portions of the documents \cite{harabagiu2001answering}. 

Why would a user take the burden to ask a complex list question? Can the user always ask a correct question? Questions evolve as they start receiving answers. 

A question comes from a distribution over words given a users mental model. When a user gains more knowledge, the mental model improves, and the distribution over words changes, which makes a user ask complex questions possibly reducing the variance of the probability distribution. 

Can users find appropriate contextual words?

If we present potential sentences, can users extract entities from them? 

We describe model editing with term relevance feedback for entity retrieval. These models can range from IR models like Rocchio, Relevance Models, Embedding based Searching Models, and Graphical Models such as Conditional Random Field (CRF). The natural way to improve a model is to feed it with more data. However, there exists situations mostly in personalized applications, where there is scarcity of training data. We explore human-centered ways of improving ML and IR models and show that with increasing number of relevance feedback on terms, we can reach the performance of an Oracle model.  


Can we simulate this idea? 

How much contextual clue is 

\section{Problem}
Entities should be matched based on a global context, whereas sentences should be matched based on a local context. There is a trade-off.

Similar entities in similar context. 

\paragraph{RQ: Does contextual information bring similar entities given the context is a sentence? }
\paragraph{ANS: Yes, at least 90\% of the entities are found in top-1000 documents}
\paragraph{RQ: How much contextual evidence should the sentence contain?}


We can take input for local context based on the sentences. 
Assumption: If a user marks a sentence that means that the contextual evidence present in that sentence is somewhat enough for the user to identify an entity. 

Does it also mean that the contextual evidence present in that entity is enough to construct a profile for that entity?
Answer: Let's assume that there are other entities like PER, LOC, ORG in that sentence. Are they enough for constructing a profile for an entity? Depends on the sentence. Most of the cases they should not be enough, and the user should be allowed to give feedback on his/her preference and there should be an interface to facilitate it. A nice way to let the user elicit her preference might be to show a set of co-occurring entities that might be of user interest. How to find those co-occurring entities? Can we construct a probability distribution over the available set of entities given the context entities, rank them and finally show the user? As the context entities are not bound by the contextual evidence given in the sentence, one possible choice is to use entity embedding and get a probability distribution over same types of entities by computing similarity. Does that go into the sentence context also? We assume that it can move into the sentence context too. 

Major target is to score a sentence.

How to score a sentence based on these inputs:
1. Entity Probability based on similarity with query entity
2. Context Matching  

So, expand query with user feedback entities, and match sentences based on that, and produce a ranked list. After that match entities with the given entity based on the user given profile. 

However, that contextual evidence might not be enough to classify an entity as the target entity, because the description of an entity from a sentence might not be too specific.

How to construct entity description? 
We can construct entity description using co-occurring entities. A person, location and/or organization can set up an

However, this can not be formulated as a supervised ML problem

The user also requires that other similar entities presented to him should be in som

The contextual evidence might be the token vector obtained from the sentence except for the entity tokens. 

We can take input on global context based on entities. 
Assumption: 

what is the sentence that best describes the topic, the entity class and contains a relevant entity?


\section{Interface Design}

We hypothesize that context words are important for entity profiling i.e. constructing a keyword based profile for a class of entities. We have seen from our previous experiments that if we include more judged sentences with the query, it improves. We need to investigate the role of context words in those sentences, by adding them one by one and assessing the performance. We can also check if the frequency of the words matter, because some words might be added multiple times in the representation and it might have an influence on the ultimate query. 

Now, the next question is how we can get the context words. The simplest answer to this question is to use pseudo relevance feedback and construct a ranked list of terms. Existing term relevance feedback based systems show words as a list or menu and let the users select words using check boxes. Our problem is challenging because with the initial query we do not get a good ranked list in the top-k retrieved documents. Hence, it is hard to decide which terms to use for constructing context profiles. So, we arrange potential contextual words in a two dimensional surface and let the users draw a line that separates the surface into four sub-regions. The top-left region would be treated as the relevant region and terms in that region would be used for query expansion. 

